NIFTY: Neural Object Interaction Fields for Guided Human Motion Synthesis

We address the problem of generating realistic 3D motions of humans interacting with objects in a scene. Our key idea is to create a neural interaction field attached to a specific object, which outputs the distance to the valid interaction manifold given a human pose as input. This interaction field guides the sampling of an object-conditioned human motion diffusion model, so as to encourage plausible contacts and affordance semantics. To support interactions with scarcely available data, we propose an automated synthetic data pipeline. For this, we seed a pre-trained motion model, which has priors for the basics of human movement, with interaction-specific anchor poses extracted from limited motion capture data. Using our guided diffusion model trained on generated synthetic data, we synthesize realistic motions for sitting and lifting with several objects, outperforming alternative approaches in terms of motion quality and successful action completion. We call our framework NIFTY: Neural Interaction Fields for Trajectory sYnthesis.

==> supp_figures/tmp-pdfcrop-6275.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{6C696B6572745F757365725F696E737472756374696F6E732E706466}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{3}


==> supp_results/baseline.tex <==


\begin{table}[h!]
    \setlength{\tabcolsep}{3pt}
    \caption{\textbf{Baseline Full Metrics.} } 
    \centering 
    \vspace{-1mm}
    \begin{adjustbox}{max width=\linewidth}
    
     \begin{tabular}{l r@{~~}r@{~~}rr@{~~}rrr} \toprule
        
                & \multicolumn{7}{r}{\textbf{Sitting}} \\
                % \midrule
        Method  & Foot                 & \% {\it D2O}          &  {\it D2O}                              & Skel.                &  \% Skel.                   & Contact               & \% Pen.  \\
                & Skating $\downarrow$ & $\le 2cm$ $\uparrow$  &  $95^\text{th}\tilde{\%}$ $\downarrow$  & Dist. $\downarrow$   & Dist.$\le 25cm$ $\uparrow$ & IoU    $\uparrow$     &  $\le 2cm$ $\uparrow$   \\
                 \midrule   
         \humanise  & 0.77 & 88.84 & 0.13 & 1.07 & 2.59 & 0.21 & 46.41\\
         \mdmOnly & 0.36 & 37.85 & 1.06 & 2.81 & 0.00 & 0.04 & 50.00 \\
         \ours (ours) & 0.47 & 99.60 & 0.00 & 0.54 & 65.94 & 0.54 & 65.40 \\
        
    \end{tabular}
    \end{adjustbox}
    
    \begin{adjustbox}{max width=\linewidth}
    
     \begin{tabular}{l s@{~~}s@{~~}ss@{~~}sss} \toprule
        
                & \multicolumn{7}{s}{\textbf{Lifting}} \\
                % \midrule
        Method  & Foot                 & \% {\it D2O}          &  {\it D2O}                              & Skel.                &  \% Skel.                   & Contact               & \% Pen.  \\
                & Skating $\downarrow$ & $\le 2cm$ $\uparrow$  &  $95^\text{th}\tilde{\%}$ $\downarrow$  & Dist. $\downarrow$   & Dist.$\le 25cm$ $\uparrow$ & IoU    $\uparrow$     &  $\le 2cm$ $\uparrow$   \\
                 \midrule
         \humanise  & 0.66 & 57.37 & 0.66 & 1.70 & 1.39 & 0.03 & 61.11\\
         \mdmOnly & 0.28 & 36.26 & 1.14 & 2.58 & 1.00 & 0.02 & 45.05 \\
        \ours (ours)  & 0.34 & 77.69 & 0.05 & 0.42 & 61.55 & 0.17 & 69.49 \\
        \midrule
    \end{tabular}
    \end{adjustbox}

  
    \label{tab:baseline_extra}
   
\end{table}

==> supp_sections/extra.tex <==


Add extra sentences of supp here.

==> supp_sections/overview.tex <==
\section{Overview}

This supplementary material provides additional context on the details of the paper along with supplemental results that were omitted due to space constraints. 
In addition to this document (\texttt{supplementary.pdf}), we also provide an HTML webpage of video results (\texttt{supplementary.html}) and \texttt{supp\_video\_source} contains all the videos in the webpage. 
\textbf{We encourage the reader to view the webpage} of qualitative results and data examples, which are best to judge the quality of motion and compare results. 
% Below we discuss the overview of the rest of the supplementary in the following sections.

In \S \ref{sec:datagen}, we discuss additional details of our data collection algorithm and evaluate data quality with a user study, while \S \ref{sec:implementation} provides details of our \ours model.  \S \ref{sec:qualitative} discusses additional qualitative results. In \S\ref{sec:quantitative}, we provide additional details on experiments from the main paper, including our baseline comparison user study in \S\ref{subsec:userstudy} and the behavior of different metrics.
\S \ref{sec:newresults} provides supplemental results to further analyze the performance of our diffusion model and interaction field. 
Finally, \S \ref{sec:failures} discusses limitations.

==> supp_sections/todo.tex <==

\begin{itemize}
  \item Writing
    \begin{itemize}
        \item 
    \end{itemize}
  \item Videos
  \item Ablations \& Results
  
\end{itemize}
